OCRia-1 Technical Report

We introduce OCRia-1, a 4B vision-language model (VLM) for document parsing that excels at preserving table structure, extracting chart data and retaining text formatting. OCRia-1 handles content that has traditionally been challenging in document parsing: merged cells and spanning headers, tables with thousands of cells, chart data, and meaningful text formatting such as bold, italics, subscripts and superscripts, preserving details needed for business-critical document analysis. At the time of this report, it achieves the highest scores on tables, charts and text formatting among the systems evaluated, including a 35B model and Mistral OCR 4.1. Its mean ParseBench score over the four dimensions we evaluate is 0.87, against 0.75 for the next-best system. We emphasize data quality and reward design in training OCRia-1. Synthetic pages provide exact ground truth for long tables and rich formatting, while real pages are transcribed using a pipeline grounded in the PDF text layer. We attribute OCRia-1's performance primarily to careful data curation that prioritizes quality and diversity over quantity. Dimension-specific rewards evaluate table reconstruction, chart-data extraction and text-formatting fidelity. We train the model on the curated data using supervised fine-tuning (SFT), then refine it through reinforcement learning with verifiable rewards (RLVR). To our knowledge, OCRia-1 is the fastest published document-parsing VLM in its class, decoding at about 4,700 tokens per second with a single request on one B200 GPU, about nine times faster than the base model on stock vLLM. This is achieved through a block-diffusion speculator, quantization and custom kernels.

==> figures/speed_systems_style.tex <==
\pgfplotsset{
  speedsys/.style={
    width=0.46\linewidth, height=4.0cm, scale only axis=false,
    xbar, bar width=7pt, bar shift=0pt, y dir=reverse,
    symbolic y coords={ocria,nemotron,hunyuan,smol,falcon}, ytick={ocria,nemotron,hunyuan,smol,falcon}, enlarge y limits=0.15,
    xmin=0, /pgf/number format/assume math mode=true,
    axis line style={LIPanelLine, line width=0.4pt},
    tick style={LIPanelLine, line width=0.4pt},
    xmajorgrids, major grid style={LIPanelLine, line width=0.3pt},
    tick label style={font=\scriptsize\sffamily, text=LIMuted},
    yticklabel style={font=\scriptsize\sffamily, text=LIInk, align=right},
    label style={font=\scriptsize\sffamily, text=LIInk},
    title style={font=\footnotesize\sffamily\bfseries, text=LIInk, yshift=-1.5mm},
    nodes near coords,
    every node near coord/.append style={font=\fontsize{6pt}{6pt}\selectfont\sffamily\bfseries, anchor=west, inner sep=1.5pt},
    clip=false,
  },
  speedsyslabels/.style={yticklabels={{\ocria{} (optimized)}, Nemotron-3.5-Parse, {HunyuanOCR-1.5 + DFlash}, SmolDocling-256M, Falcon-OCR bf16}},
  speedsysocria/.style={fill=LIBlue, draw=none, every node near coord/.append style={text=LIBlue}},
  speedsysother/.style={fill=LIMuted, draw=none, every node near coord/.append style={text=LIMuted}},
}

